Discrete Geodesic Nets for Modeling Developable Surfaces

We present a discrete theory for modeling developable surfaces as quadrilateral meshes satisfying simple angle constraints. The basis of our model is a lesser known characterization of developable surfaces as manifolds that can be parameterized through orthogonal geodesics. Our model is simple, local, and, unlike previous works, it does not directly encode the surface rulings. This allows us to model continuous deformations of discrete developable surfaces independently of their decomposition into torsal and planar patches or the surface topology. We prove and experimentally demonstrate strong ties to smooth developable surfaces, including a theorem stating that every sampling of the smooth counterpart satisfies our constraints up to second order. We further present an extension of our model that enables a local definition of discrete isometry. We demonstrate the effectiveness of our discrete model in a developable surface editing system, as well as computation of an isometric interpolation between isometric discrete developable shapes.

==> 98-acks.tex <==
\section*{Acknowledgments}
The authors would like to thank Shahar Kovalsky for providing the source code for AQP and for illuminating discussions, and the anonymous
reviewers for their useful comments and suggestions.
This work was supported in part by the ERC grant iModel (StG-2012-306877), a gift from Adobe, and Courant Institute's faculty start-up funding.
